HUE: Pretrained Model and Dataset for Understanding Hanja Documents of Ancient Korea

Historical records in Korea before the 20th century were primarily written in Hanja, an extinct language based on Chinese characters and not understood by modern Korean or Chinese speakers. Historians with expertise in this time period have been analyzing the documents, but that process is very difficult and time-consuming, and language models would significantly speed up the process. Toward building and evaluating language models for Hanja, we release the Hanja Understanding Evaluation dataset consisting of chronological attribution, topic classification, named entity recognition, and summary retrieval tasks. We also present BERT-based models continued training on the two major corpora from the 14th to the 19th centuries: the Annals of the Joseon Dynasty and Diaries of the Royal Secretariats. We compare the models with several baselines on all tasks and show there are significant improvements gained by training on the two corpora. Additionally, we run zero-shot experiments on the Daily Records of the Royal Court and Important Officials (DRRI). The DRRI dataset has not been studied much by the historians, and not at all by the NLP community.

==> texes/_5_experiments_deprecated.tex <==


% \begin{table}[!]
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|r|r|r}
% \hline
% \textbf{Models}             & \multicolumn{1}{c|}{\textbf{\# of <unk>}} & \multicolumn{1}{c|}{\textbf{\# of tokens}} & \multicolumn{1}{c}{\textbf{ratio}} \\ \hline
% \textbf{AnchiBERT}          & 1,860,269                               & 211,471,872                                & 0.88\%                             \\
% \textbf{mBERT}              & 1,601,173                               & 211,471,872                                & 0.76\%                             \\
% \textbf{AnchiBERT +AJD/DRS} & 89,271                                  & 211,471,872                                & 0.04\%                             \\
% \textbf{mBERT + AJD/DRS}    & 89,271                                  & 211,471,872                                & 0.04\%                             \\ \hline
% \end{tabular}
% }
% \caption{Unknown Token Ratio in Each PLM}
% \label{tab:unk_token}
% \end{table}

% \begin{table}[!]
% \centering
% \begin{tabular}{l|r}
% \hline
% Models             & \multicolumn{1}{c}{ratio} \\ \hline
% AnchiBERT          & 0.88\%                    \\
% mBERT              & 0.76\%                    \\ \hline
% AnchiBERT +AJD/DRS & 0.04\%                    \\
% mBERT + AJD/DRS    & 0.04\%                    \\ \hline
% \end{tabular}
% \caption{Unknown Token Ratio in Each PLM}
% \label{tab:unk_token}
% \end{table}

% \begin{table}[!]
% \centering
% \begin{tabular}{l|r}
% \hline
% Models              & \multicolumn{1}{c}{ratio} \\ \hline
% AnchiBERT           & 0.88\%                    \\
% +AJD/DRS            & 0.04\%                    \\ \hline
% mBERT               & 0.76\%                    \\
% +AJD/DRS           & 0.04\%                    \\ \hline
% \end{tabular}
% \caption{Unknown Token Ratio in Each PLM}
% \label{tab:unk_token_1}
% \end{table}


\subsection{Overall Results}

% \begin{table*}[!]
% \centering
% \begin{tabular}{l|c|ccc|c|c}
% \hline
%                     & \multirow{2}{*}{\textbf{King}} & \multicolumn{3}{c|}{\textbf{Topic}}              & \multirow{2}{*}{\textbf{NER}} & \multirow{2}{*}{\textbf{Summarization}} \\
% \textbf{}           &                                & Div1              & Div2              & Div3              &                               &                                         \\
% Model               & F1                             & F1                & F1                & F1                & F1                            & mrr                                     \\ \hline
% BERT not pretrained & 54.26                          & 68.91             & 61.52             & 46.22             & 89.40                         &                                         \\
% AnchiBERT           & 75.74                          & 85.81             & 75.22             & \underline{48.86} & 90.30                         & 67.06                                   \\
% mBERT               & 75.29                          & 79.59             & 76.46             & 46.19             & 88.57                         &                                         \\
% AnchiBERT + AJD/DRS & \textbf{79.33}                 & \textbf{88.33}    & \textbf{78.10}    & \textbf{48.86}    & \textbf{90.42}                &                                         \\
% mBERT + AJD/DRS     & \underline{77.77}              & \underline{87.13} & \underline{77.84} & 48.61             & \underline{90.16}             & 73.88                                   \\ \hline
% \end{tabular}
% \caption{Evaluation Results for our PLMs on Hanja Benchmark}
% \label{tab:overall}
% \end{table*}

% \begin{table*}[!]
% \centering
% \begin{tabular}{l|c|cc|c|c}
% \hline
%                     & \multirow{2}{*}{\textbf{King}} & \multicolumn{2}{c|}{\textbf{Topic}}   & \multirow{2}{*}{\textbf{NER}} & \multirow{2}{*}{\textbf{Summarization}} \\
% \textbf{}           &                                & Major             & Minor             &                               &                                         \\
% Model               & F1                             & F1                & F1                & F1                            & mrr                                     \\ \hline
% BERT not pretrained & 54.26                          & 68.91             & 61.52             & 89.40                         & 52.85                                   \\
% AnchiBERT           & 75.74                          & 85.81             & 75.22             & 90.30                         & 67.92                                   \\
% mBERT               & 75.29                          & 79.59             & 76.46             & 88.57                         & 67.06                                   \\
% AnchiBERT + AJD/DRS & \textbf{79.33}                 & \textbf{88.33}    & \textbf{78.10}    & \textbf{90.42}                & \textbf{74.29}                          \\
% mBERT + AJD/DRS     & \underline{77.77}              & \underline{87.13} & \underline{77.84} & \underline{90.16}             & \underline{73.88}                       \\ \hline
% \end{tabular}
% \caption{Evaluation Results for our PLMs on Hanja Benchmark}
% \label{tab:overall}
% \end{table*}

\begin{table*}[!]
\centering
\begin{tabular}{l|c|cc|c|c}
\hline
                    & \textbf{KP}                    & \multicolumn{2}{c|}{\textbf{TC}}      & \textbf{NER}                  & \textbf{Summarization}                  \\
\textbf{}           &                                & \textbf{Major}    & \textbf{Minor}    &                               &                                         \\
Model               & F1                             & F1                & F1                & F1                            & mrr                                     \\ \hline
BERT not pretrained & 54.26                          & 68.91             & 61.52             & 89.40                         & 52.85                                   \\
AnchiBERT           & 75.74                          & 85.81             & 75.22             & 90.30                         & 67.92                                   \\
mBERT               & 75.29                          & 79.59             & 76.46             & 88.57                         & 67.06                                   \\
AnchiBERT + AJD/DRS & \textbf{79.33}                 & \textbf{88.33}    & \textbf{78.10}    & \textbf{90.42}                & \textbf{74.29}                          \\
mBERT + AJD/DRS     & \underline{77.77}              & \underline{87.13} & \underline{77.84} & \underline{90.16}             & \underline{73.88}                       \\ \hline
\end{tabular}
\caption{Evaluation Results for our PLMs on Hanja Benchmark}
\label{tab:overall}
\end{table*}

% We also set BERT without any pretraining as a baseline model to inspect whether pretraining language models on hanja domain data is critical in predicting preliminary attributes.
We present all results in Table \ref{tab:overall}, and it gives some observations. First, BERT without pretraining shows the poorest results among all tasks. It indicates that all these benchmark tasks require domain-specific data. Also, the existing PLMs (AnchiBERT and mBERT) show a better result than BERT without any \jiho{additional} pretraining, but the models re-trained on hanja documents achieve the best performance among all tasks.

\subsection{King Prediction}

% \begin{table*}[!]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccccc|ccccc}
% \hline
% \textbf{}           & \multicolumn{5}{c|}{\textbf{Default}}                                              & \multicolumn{5}{c}{\textbf{Entity Masked}}                                         \\
% Model               & acc            & F1             & pre            & rec            & qwk            & acc            & F1             & pre            & rec            & qwk            \\ \hline
% BERT not pretrained & 56.59          & 54.26          & 55.08          & 56.59          & 87.09          & 75.43          & 75.07          & 75.73          & 75.43          & 92.61          \\
% AnchiBERT           & 76.31          & 75.74          & 76.45          & 76.31          & 93.99          & 82.77          & 82.44          & 82.71          & 82.77          & 95.66          \\
% mBERT               & 76.02          & 75.29          & 75.80          & 76.02          & 93.76          & 83.56          & 83.44          & 83.80          & 83.56          & 95.56          \\
% AnchiBERT + AJD/DRS & \textbf{79.50} & \textbf{79.33} & \textbf{80.06} & \textbf{79.50} & \textbf{95.46} & \textbf{83.73} & \textbf{83.58} & 84.31          & \textbf{83.73} & 96.16          \\
% mBERT + AJD/DRS     & 77.99          & 77.78          & 78.92          & 77.99          & 95.04          & 83.63          & 83.57          & \textbf{84.33} & 83.63          & \textbf{96.43} \\ \hline
% \end{tabular}
% }
% \caption{Evaluation Results for our PLMs on King Prediction}
% \label{tab:king}
% \end{table*}

% \begin{table*}[!]
% \centering
% \begin{tabular}{l|ccccc}
% \hline
% \textbf{}           & \multicolumn{5}{c}{\textbf{Default} $_\text{Difference on Entity Masked}$}                                                                         \\
% Model               & acc                      & F1                       & pre                      & rec                      & qwk                      \\ \hline
% BERT not pretrained & 56.59 $_{+18.83}$         & 54.26 $_{+20.81}$         & 55.08 $_{+20.65}$         & 56.59 $_{+18.83}$         & 87.09 $_{+5.51}$          \\
% AnchiBERT           & 76.31 $_{+6.46}$          & 75.74 $_{+6.71}$          & 76.45 $_{+6.26}$          & 76.31 $_{+6.46}$          & 93.99 $_{+1.67}$          \\
% mBERT               & 76.02 $_{+7.54}$          & 75.29 $_{+8.15}$          & 75.80 $_{+8.00}$          & 76.02 $_{+7.54}$          & 93.76 $_{+1.80}$          \\
% AnchiBERT + AJD/DRS & \textbf{79.50 $_{+4.23}$} & \textbf{79.33 $_{+4.25}$} & \textbf{80.06 $_{+4.26}$} & \textbf{79.50 $_{+4.23}$} & \textbf{95.46 $_{+0.70}$} \\
% mBERT + AJD/DRS     & 77.99 $_{+5.64}$          & 77.78 $_{+5.80}$          & 78.92 \textbf{$_{+5.41}$} & 77.99 $_{+5.64}$          & 95.04 \textbf{$_{+1.39}$} \\ \hline
% \end{tabular}
% \caption{Evaluation Results for our PLMs on King Prediction}
% \label{tab:king}
% \end{table*}

% \begin{table*}[!]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|cc|cc|cc|cc}
% \hline
% \textbf{}           & \multicolumn{2}{c|}{acc}              & \multicolumn{2}{c|}{F1}               & \multicolumn{2}{c|}{pre}              & \multicolumn{2}{c|}{rec}              & \multicolumn{2}{c}{qwk}               \\
% Model               & Non               & Mask              & Non               & Mask              & Non               & Mask              & Non               & Mask              & Non               & Mask              \\ \hline
% BERT not pretrained & 56.59             & 75.43             & 54.26             & 75.07             & 55.08             & 75.73             & 56.59             & 75.43             & 87.09             & 92.61             \\
% AnchiBERT           & 76.31             & 82.77             & 75.74             & 82.44             & 76.45             & 82.71             & 76.31             & 82.77             & 93.99             & 95.66             \\
% mBERT               & 76.02             & 83.56             & 75.29             & 83.44             & 75.80             & 83.80             & 76.02             & 83.56             & 93.76             & 95.56             \\
% AnchiBERT + AJD/DRS & \textbf{79.50}    & \textbf{83.73}    & \textbf{79.33}    & \textbf{83.58}    & \textbf{80.06}    & \underline{84.31} & \textbf{79.50}    & \textbf{83.73}    & \textbf{95.46}    & \underline{96.16} \\
% mBERT + AJD/DRS     & \underline{77.99} & \underline{83.63} & \underline{77.78} & \underline{83.57} & \underline{78.92} & \textbf{84.33}    & \underline{77.99} & \underline{83.63} & \underline{95.04} & \textbf{96.43}    \\ \hline
% \end{tabular}
% }
% \caption{Evaluation Results for our PLMs on King Prediction}
% \label{tab:king}
% \end{table*}

\begin{table*}[!]
\centering
% \resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccccc}
\hline
                      & acc               & F1                & pre               & rec               & qwk               \\ \hline
BERT not pretrained   & 56.59             & 54.26             & 55.08             & 56.59             & 87.09             \\
AnchiBERT             & 76.31             & 75.74             & 76.45             & 76.31             & 93.99             \\
mBERT                 & 76.02             & 75.29             & 75.80             & 76.02             & 93.76             \\
AnchiBERT + AJD/DRS   & \textbf{79.50}    & \textbf{79.33}    & \textbf{80.06}    & \textbf{79.50}    & \textbf{95.46}    \\
mBERT + AJD/DRS       & \underline{77.99} & \underline{77.78} & \underline{78.92} & \underline{77.99} & \underline{95.04} \\ \hline
\end{tabular}
% }
\caption{Evaluation Results for our PLMs on King Prediction}
\label{tab:king}
\end{table*}


% \begin{figure*}[!]
%     \centering
%     \subfloat[\centering BERT without pretraining]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_BERT-not-pretrained.png}}
%     \qquad
%     \subfloat[\centering AnchiBERT]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_AnchiBERT.png}}
%     \qquad
%     \subfloat[\centering mBERT]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_mBERT.png}}
%     \qquad
%     \subfloat[\centering AnchiBERT + AJD/DRS]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_AnchiBERT-ajd+sjw-50.png}}
%     \qquad
%     \subfloat[\centering mBERT + AJD/DRS]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_mBERT-ajd+sjw-50.png}}
%     \qquad
%     \caption{Confusion Matrix for King Prediction}
%     \label{fig:conf_mtrx}
% \end{figure*}

% \begin{figure*}[!]
%     \centering
%     \subfloat[\centering BERT without pretraining]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_BERT-not-pretrained-logscale.png}}
%     \qquad
%     \subfloat[\centering AnchiBERT]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_AnchiBERT-logscale.png}}
%     \qquad
%     \subfloat[\centering mBERT]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_mBERT-logscale.png}}
%     \qquad
%     \subfloat[\centering AnchiBERT + AJD/DRS]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_AnchiBERT-ajd+sjw-50-logscale.png}}
%     \qquad
%     \subfloat[\centering mBERT + AJD/DRS]{\includegraphics[width=2.5cm]{figures/confusionmatrix_king-prediction_mBERT-ajd+sjw-50-logscale.png}}
%     \qquad
%     \caption{Log-Scale Confusion Matrix for King Prediction}
%     \label{fig:conf_mtrx}
% \end{figure*}

% \begin{figure*}[!
%     \centering
%     \subfloat[\centering BERT without pretraining]{\includegraphics[width=2.5cm]{figures/abs_diff_per_class-BERT-not-pretrained.png}}
%     \qquad
%     \subfloat[\centering AnchiBERT]{\includegraphics[width=2.5cm]{figures/abs_diff_per_class-AnchiBERT.png}}
%     \qquad
%     \subfloat[\centering mBERT]{\includegraphics[width=2.5cm]{figures/abs_diff_per_class-mBERT.png}}
%     \qquad
%     \subfloat[\centering AnchiBERT + AJD/DRS]{\includegraphics[width=2.5cm]{figures/abs_diff_per_class-AnchiBERT-ajd+sjw-50.png}}
%     \qquad
%     \subfloat[\centering mBERT + AJD/DRS]{\includegraphics[width=2.5cm]{figures/abs_diff_per_class-mBERT-ajd+sjw-50.png}}
%     \qquad
%     \caption{Mean Absolute Difference per Class for King Prediction}
%     \label{fig:conf_mtrx}
% \end{figure*}

% \begin{figure}[!ht]
%     \centering
%     \subfigure[Log-scale Confusion Matrix]{\includegraphics[width=0.8\columnwidth]{final_figures/conf_mtrx_log.pdf}}
%     \subfigure[Mean Absolute Difference per King]{\includegraphics[width=0.8\columnwidth]{final_figures/mean_abs_diff.pdf}}
%     \caption{Classification Results with AnchiBERT + AJD/DRS}
%     \label{fig:conf_diff}
% \end{figure}

Table \ref{tab:king} shows the evaluation results on KP, and the models show similar tendencies to the overall results where re-trained AnchiBERT outperforms other models. 
% Figure \ref{fig:conf_diff} (a) shows log-scale confusion matrix on AnchiBERT re-trained on AJD and DRS, and indicates that the model's predictions in which king reign the document was written in a reliable level, which can also be inferred from Figure \ref{fig:conf_diff} (b), the mean absolute difference per kings. We measure the Quadratic Weighted Kappa score (QWK score) as metrics that treat each label hierarchically. The right side of Table \ref{tab:king} shows the evaluation results of the KP in the same settings, but all named entities (both person and location entities) in the input sources are masked. Compared to the default settings, all models show significant improvements, which does not mask named entities.

% Each bar in Figure \ref{fig:conf_diff} (b) indicates the mean absolute difference per class, and the line graph means the number of samples in the test set. The results of the last two Emperors Gojong and Sunjong are remarkable in that the model rarely gets confused with those two labels to others and tends not to fail. We believe that this is because our model learns the difference between those two records and the others in terms of historical view and get cues to distinguish them. Most of the classes achieved the difference around one, except for the first King Taejo and the second King Jeongjong, whose difference is almost doubled. We hypothesize that this is mainly because there are too small examples in those classes. A similar tendency where the more samples are, the less mean absolute difference be has been observed in other classes. Also, the writing format of AJD had settled down from the third King Taejong, and the unstructured records might confuse models to predict the exact dates.


\subsection{Topic Classification}

\begin{figure}[!]
    \centering
    \subfigure{\includegraphics[width=\columnwidth]{final_figures/legend_2lines.pdf}}
    \addtocounter{subfigure}{-1}
    \subfigure[\centering Div 1 (4 classes)]{\includegraphics[width=0.45\columnwidth]{final_figures/topic-div1.pdf}}
    \subfigure[\centering Div 2 (106 classes)]{\includegraphics[width=0.45\columnwidth]{final_figures/topic-div2.pdf}}
    % \subfigure[\centering Div 3 (199 classes)]{\includegraphics[width=0.3\linewidth]{final_figures/topic-div3.pdf}}
    \caption{ROC Curve and AUC for Topic Classification. Each value in the plot indicates the AUC score.}
    \label{fig:roc_auc}
\end{figure}

% \begin{figure*}[!]
%     \centering
%     \subfigure{\includegraphics[width=\linewidth]{final_figures/legend.pdf}}
%     \addtocounter{subfigure}{-1}
%     \subfigure[\centering Div 1 (4 classes)]{\includegraphics[width=0.3\linewidth]{final_figures/topic-div1.pdf}}
%     \subfigure[\centering Div 2 (106 classes)]{\includegraphics[width=0.3\linewidth]{final_figures/topic-div2.pdf}}
%     % \subfigure[\centering Div 3 (199 classes)]{\includegraphics[width=0.3\linewidth]{final_figures/topic-div3.pdf}}
%     \caption{ROC Curve and AUC for Topic Classification. Each value in the plot indicates the AUC score.}
%     \label{fig:roc_auc}
% \end{figure*}

\begin{table*}[!]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\hline
\textbf{}           & \multicolumn{5}{c|}{\textbf{Major (4 classes)}}                                                   & \multicolumn{5}{c}{\textbf{Minor (106 classes)}}                                                  \\
Model               & acc               & F1                & pre               & rec               & ham               & acc               & F1                & pre               & rec               & ham               \\ \hline
BERT not pretrained & 68.52             & 68.91             & 74.82             & 70.65             & 79.04             & 26.48             & 61.29             & 54.86             & 84.59             & 42.45             \\
AnchiBERT           & 68.99             & 85.81             & 85.24             & 88.44             & 83.00             & 31.47             & 69.30             & 61.63             & 90.26             & 51.63             \\
mBERT               & 56.78             & 79.59             & 77.60             & 87.78             & 73.64             & \underline{32.85} & 70.01             & 62.17             & 90.84             & \underline{54.28} \\
AnchiBERT + AJD/DRS & \textbf{70.48}    & \textbf{88.33}    & \textbf{86.61}    & \textbf{92.71}    & \textbf{84.80}    & 31.77             & \textbf{72.07}    & \textbf{64.87}    & \underline{91.24} & 52.25             \\
mBERT + AJD/DRS     & \underline{69.15} & \underline{87.13} & \underline{85.48} & \underline{91.36} & \underline{83.81} & \textbf{33.96}    & \underline{71.28} & \underline{63.50} & \textbf{91.56}    & \textbf{55.91}    \\ \hline
\end{tabular}
}
\caption{Evaluation Results for our PLMs on Topic Classification}
\label{tab:topic}
\end{table*}

% \begin{table*}[!]
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|ccccc|ccccc|ccccc}
% \hline
% \textbf{}           & \multicolumn{5}{c|}{\textbf{Div1 (4 classes)}}                                                    & \multicolumn{5}{c|}{\textbf{Div2 (106 classes)}}                                                  & \multicolumn{5}{c}{\textbf{Div3 (199 classes)}}                                    \\
% Model               & acc               & F1                & pre               & rec               & ham               & acc               & F1                & pre               & rec               & ham               & acc               & F1                & pre               & rec               & ham            \\ \hline
% BERT not pretrained & 68.52             & 68.91             & 74.82             & 70.65             & 79.04             & 26.48             & 61.29             & 54.86             & 84.59             & 42.45             & \underline{21.54} & 46.22             & 34.32             & 91.23             & 34.65          \\
% AnchiBERT           & 68.99             & 85.81             & 85.24             & 88.44             & 83.00             & 31.47             & 69.30             & 61.63             & 90.26             & 51.63             & 20.67             & \underline{48.86} & \underline{36.76} & 91.89             & \underline{35.23} \\
% mBERT               & 56.78             & 79.59             & 77.60             & 87.78             & 73.64             & \underline{32.85} & 70.01             & 62.17             & 90.84             & \underline{54.28} & 19.80             & 46.19             & 34.43             & 90.77             & 32.54          \\
% AnchiBERT + AJD/DRS & \textbf{70.48}    & \textbf{88.33}    & \textbf{86.61}    & \textbf{92.71}    & \textbf{84.80}    & 31.77             & \textbf{72.07}    & \textbf{64.87}    & \underline{91.24} & 52.25             & \textbf{22.05}    & \textbf{48.86}    & \textbf{36.77}    & \underline{92.54} & \textbf{36.10} \\
% mBERT + AJD/DRS     & \underline{69.15} & \underline{87.13} & \underline{85.48} & \underline{91.36} & \underline{83.81} & \textbf{33.96}    & \underline{71.28} & \underline{63.50} & \textbf{91.56}    & \textbf{55.91}    & 19.71             & 48.61             & 36.31             & \textbf{92.90}    & 34.50          \\ \hline
% \end{tabular}
% }
% \caption{Evaluation Results for our PLMs on Topic Classification}
% \label{tab:topic}
% \end{table*}

Table \ref{tab:topic} shows the evaluation results of topic classification tasks on all three divisions, and Figure \ref{fig:roc_auc} gives ROC curves and AUC values of each model on each task. Since TC is a multi-label classification whose example might have multiple labels as the answer, we measure Hamming score along with accuracy. In this case, accuracy is the exact match score, and the hamming score is the accuracy of subset matched, $\mid T \cap P \mid / \mid T \cup P \mid$, where $T$ is set of true labels and $P$ is set of predicted labels \cite{Godbole2004hammingscore}. For the evaluation results in Table \ref{tab:topic}, we find and set the best threshold to each label by Youden's index. All pretrained models outperform BERT without pretraining, and two LMs re-trained on hanja documents show the best performances.

Table \ref{tab:topic} shows results with all metrics except for recall drops if it goes to detailed division, while recall in all divisions achieves around 90\%. It indicates that the threshold is too low and models tends to predict plausible topics as many as they can, which might be solved by controlling the threshold. This is probably due to the meaning overlaps in minor categories. For instance, there are minor categories such as revenue, finance, general price level, and commerce are the sub-categories of economy in the major categories, whose use case cannot be strictly distinguished. It would be more appropriate in this case to provide all plausible topics roughly rather than suggesting the one only with high certainty.

\subsection{Named Entity Recognition}

\begin{table*}[!]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc|ccc|ccc}
\hline
\textbf{}           & \multicolumn{4}{c|}{\textbf{Overall}}                                         & \multicolumn{3}{c|}{\textbf{Person}}                      & \multicolumn{3}{c}{\textbf{Location}}                     \\
Model               & acc               & F1                & pre               & rec               & F1                & pre               & rec               & F1                & pre               & rec               \\ \hline
BERT not pretrained & 98.67             & 89.40             & 90.58             & 88.25             & 92.13             & 93.98             & 90.36             & 87.10             & 87.76             & 86.46             \\
AnchiBERT           & \underline{98.72} & 90.30             & \underline{90.98} & 89.62             & \underline{93.13} & \underline{94.47} & 91.83             & \underline{87.91} & \underline{88.08} & \underline{87.75} \\
mBERT               & 98.52             & 88.57             & 89.52             & 87.64             & 91.63             & 93.60             & 89.74             & 86.02             & 86.18             & 85.85             \\
AnchiBERT + AJD/DRS & \textbf{98.76}    & \textbf{90.42}    & \textbf{91.31}    & \underline{89.55} & \textbf{93.28}    & \textbf{94.77}    & \underline{91.84} & \textbf{88.01}    & \textbf{88.43}    & 87.59             \\
mBERT + AJD/DRS     & 98.69             & \underline{90.16} & 90.36             & \textbf{89.95}    & 92.83             & 93.51             & \textbf{92.17}    & 87.90             & 87.74             & \textbf{88.06}    \\ \hline
\end{tabular}
}
\caption{Evaluation Results for our PLMs on Named Entity Recognition}
\label{tab:ner}
\end{table*}

Table \ref{tab:ner} shows the evaluation results of NER, which indicates similar trends to the overall benchmark tasks with a small gap among models including BERT without pretraining. It implies that NER in hanja documents is a comparably easy task. This might result from certain patterns in named entities in hanja. Most of the person entities are 3 letters and start with the common character (family name), and most of the location entities end with the common character meaning locations or buildings. All models tend to predict person entities better than location entities.

\subsection{Summarization}

\begin{table}[!]
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc}
\hline
Model               & mrr               & Top-1             & Top-10            \\ \hline
BM25                & 29.87             & 25.58             & 33.98             \\
BERT not pretrained & 52.85             & 99.20             & 99.64             \\
AnchiBERT           & 67.92             & 99.20             & \underline{99.85} \\
mBERT               & 67.06             & 99.32             & 99.50             \\
AnchiBERT + AJD/DRS & \textbf{74.29}    & \textbf{99.64}    & \textbf{99.91}    \\
mBERT + AJD/DRS     & \underline{73.88} & \underline{99.44} & 99.59             \\ \hline
\end{tabular}
}
\caption{Evaluation Results for our PLMs on Summairzation}
\label{tab:summarization}
\end{table}


Table \ref{tab:summarization} shows Mean Reciprocal Rank (MRR), Top-1, and Top-10 accuracy of our PLMS on summarization task. All fine-tuned BERT-based re-rankers outperform BM25, mostly retrieving the ground truth answer at the first trial. It implies that BERT-based re-rankers might be exploited for retrieving relevant documents from different chronicles in terms of written style or contents.


\subsection{Zero-shot Experiment}

\begin{table*}[!]
% \small
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc|ccc}
\hline
                    & \multicolumn{3}{c|}{\textbf{KP}}                          & \multicolumn{3}{c|}{\textbf{NER (Person)}}                & \multicolumn{3}{c}{\textbf{NER (Location)}}                \\ 
Model               & F1                & pre               & rec               & F1                & pre               & rec               & F1                & pre               & rec               \\ \hline
BERT not pretrained & 26.94             & 27.68             & 26.23             & 68.50             & 63.27             & 70.52             & 39.86             & 39.31             & 40.45             \\
AnchiBERT           & 30.65             & 34.25             & \underline{27.73} & 71.85             & 60.97             & 78.37             & 77.23             & \textbf{85.65}    & 70.50             \\
mBERT               & 32.19             & 28.80             & \textbf{28.02}    & 72.08             & 61.10             & 80.95             & \textbf{83.36}    & 83.03             & \textbf{83.68}    \\
AnchiBERT + AJD/DRS & \textbf{35.85}    & \textbf{59.62}    & 25.63             & \underline{82.86} & \underline{68.01} & \textbf{92.60}    & \underline{76.53} & \underline{84.74} & \underline{75.95} \\
mBERT + AJD/DRS     & \underline{35.28} & \underline{48.67} & 27.67             & \textbf{88.48}    & \textbf{73.71}    & \underline{90.91} & 72.08             & 81.29             & 75.35             \\ \hline
\end{tabular}
}
\caption{Zero-shot Experimental Results on DRRI}
\label{tab:zero-shot}
\end{table*}

Table \ref{tab:zero-shot} shows experimental results with KP and NER on DRRI which are not used in both re-training PLMS and fine-tuning. All models perform comparably well on the both tasks, regarding that random model will achieve approximately 3.70\% performances with 27 classes in KP. Also, all models in KP commonly show high precision which might be due to the monotonous and redundant phrases in the veritable records. There was similar trends compared to the Table \ref{tab:king}, but the gap among models was notably emphasized in the zero-shot settings. This results imply that our KP models might be exploited for the written ages prediction of unseen documents in anthology with a reliable level.

Our models outperform others on NER achieving absolutely high performances, considering that entity maps between AJD and DRRI do not match strictly. Interestingly, all models tend to predict location entities better than person entities which is the opposite result compared to the original NER on AJD. It is probably due to the characteristics of each entity, where location entities are all commonly used in nationwide while person entity might differ by situation. We present that our models trained on the corpora of the Joseon dynasty provide reliable results on unseen records, implying that our model can be exploited in the low-resourced documents.
